Core Discovery in Hidden Graphs

Massive network exploration is an important research direction with many applications. In such a setting, the network is, usually, modeled as a graph $G$, whereas any structural information of interest is extracted by inspecting the way nodes are connected together. In the case where the adjacency matrix or the adjacency list of $G$ is available, one can directly apply graph mining algorithms to extract useful knowledge. However, there are cases where this is not possible because the graph is \textit{hidden} or \textit{implicit}, meaning that the edges are not recorded explicitly in the form of an adjacency representation. In such a case, the only alternative is to pose a sequence of \textit{edge probing queries} asking for the existence or not of a particular graph edge. However, checking all possible node pairs is costly (quadratic on the number of nodes). Thus, our objective is to pose as few edge probing queries as possible, since each such query is expected to be costly. In this work, we center our focus on the \textit{core decomposition} of a hidden graph. In particular, we provide an efficient algorithm to detect the maximal subgraph of $S_k$ of $G$ where the induced degree of every node $u \in S_k$ is at least $k$. Performance evaluation results demonstrate that significant performance improvements are achieved in comparison to baseline approaches.

==> figs/hiddencoreexample.tex <==
% Generated with LaTeXDraw 2.0.8
% Tue Oct 10 22:05:55 EEST 2017
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-1.57125)(2.9775,1.61125)
\definecolor{color28b}{rgb}{0.10588235294117647,0.0784313725490196,0.0784313725490196}
\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color28b](0.91,0.03875){0.21}
\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color28b](0.65,-1.06125){0.21}
\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color28b](2.41,0.01875){0.21}
\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color28b](2.57,-1.36125){0.21}
\psline[linewidth=0.04cm](0.88,0.06875)(0.66,-1.05125)
\psline[linewidth=0.04cm](0.88,0.02875)(2.4,0.00875)
\psline[linewidth=0.04cm](2.44,0.02875)(2.62,-1.35125)
\psline[linewidth=0.04cm](0.62,-1.07125)(2.56,-1.33125)
\psline[linewidth=0.04cm](0.66,-1.09125)(2.48,-0.01125)
\psline[linewidth=0.04cm](0.94,0.00875)(2.68,-1.51125)
\usefont{T1}{ppl}{m}{n}
\rput(0.295625,-0.82125){4}
\usefont{T1}{ppl}{m}{n}
\rput(0.4434375,0.01875){2}
\usefont{T1}{ppl}{m}{n}
\rput(2.7664063,0.23875){3}
\usefont{T1}{ppl}{m}{n}
\rput(2.8248436,-1.00125){5}
\pscircle[linewidth=0.04,dimen=outer,fillstyle=solid,fillcolor=color28b](0.21,1.13875){0.21}
\psline[linewidth=0.04cm](0.2,1.12875)(0.96,-0.01125)
\usefont{T1}{ppl}{m}{n}
\rput(0.458125,1.41875){1}
\end{pspicture} 
}



==> proposed2.tex <==
%\begin{flushleft}\textbf{GSOE output: \textit{TOP} list}\end{flushleft}
%GSOE requires only one user input, an integer K which is the number of top-K degree nodes that user asks for. The rationale of GSOE is based on the proper selection of the source node. Given that source node has been selected, the next concern is to find a suitable destination node to perform a probing between them. If the probing result is 'E', GSOE searches for a new source node. Otherwise, GSOE keeps source node unchanged and starts searching for the next suitable destination to probe. The proper selection of source and destination nodes makes nodes with higher degree to perform more probings in less time than those with lower degree. As a result, their actual degree is revealed earlier without performing probings between nodes with lower degree. Once the algorithm estimates that a node belongs to top-K degree nodes it pushes the node to the \textit{TOP} list. This list holds the top-K degree nodes in descending order from the one with the highest degree till the k-th highest degree node. Apparently \textit{TOP} is the final outcome of GSOE. 





\begin{flushleft}\textbf{Node-level data structures and properties}\end{flushleft}
During G-SOE probings, every node in graph G(V,E) maintains 3 counters and a list:\\~\\
\textit{\textbf{s}}, an nonnegative integer counter. It holds the number of 's'olid probing queries that the node participated as either source or destination. It is initialized to zero.\\~\\
\textit{\textbf{e}}, an nonnegative integer counter. It holds the number of 'e'mpty probing queries that the node participated as either source or destination. It is initialized to zero.\\~\\
  \textit{\textbf{state}} is a new parameter that does not exist in the original SOE. It is a non positive integer counter. Whenever an empty probing comes up both source and destination nodes decrease their state value by one. It is not increased at solid probings! Moreover G-SOE increases by one the nodes that have negative state at the end of each round.\textit{state} is initialized to zero.\\~\\  



The following Lemma applies to every undirected hidden graph G(V,E) where $\left|V\right|$=N\newline
\textit{\textbf{Lemma 1:}} $\forall v\in V:deg(v)=v.s \Leftrightarrow v.s+v.e = N-1$\\~\\
The maximum degree a node could have in a graph G(V,E) equals to N-1, where $\left|V\right|$=N. Consequently, if we want to find the actual degree of a node in a hidden graph then N-1 probing queries are required, independent of the probings' directions. Since s and e counters hold the number of solid and empty probings of a node, Lemma 1 implies that s counter is equal to the actual degree if and only if all possible probings have been performed for this node.\\
\textit{\textbf{SegmentList}} is a list of logN triplets called Segments. Each triplet consists of a counter $c$ with an initial N/logN value and two empty lists, $eList$ and $sList$ as shown in Fig3. \textit{SegmentList} is required to find the proper destination node, given that the source node has already been selected. It is used right before (Search stage) and right after (Update stage) the probing. \newline
\textit{Search stage:} Every Segment refers to a segment of N/logN destination candidates. i.e 1st Segment refers to [1,N/(logN-1)] candidates, 2nd Segment refers to [N/(logN-1),2N/(logN-1)] candidates.. e.t.c. GSOE starts searching the source's \textit{SegmentList} in order to find the first Segment with non zero counter. Once a Segment is found, its counter $c$ is decreased by one and the Search stage starts. The first node in the Segment that is not included in the Segment's eList or sList is the proper destination node to perform a probing with the selected source node.\newline
\textit{Update stage:} Once the probing between source and destination node is performed, both nodes' \textit{SegmentLists} are updated (Update stage) with the probing result. In case of source node, GSOE updates the Segment where destination node came from. If the probing result was solid the destination node is added to Segment's sList, otherwise it is added to eList. In case of destination node, GSOE updates destination's SegmentList as if source and destination interchanged their roles. Destination node act as source and searches its \textit{SegmentList} in order to find the Segment that refers to source. Depending one the probing result it adds source node to either sList or eList. The update of \textit{SegmentLists} helps G-SOE to avoid re-probing between the same nodes.\newline

\begin{figure}[H]
\begin{center}
\vspace*{-7ex}\includegraphics[scale=0.8]{figs/SegmentList.eps}
\end{center}
\caption{The structure of a SegmentList during initialization.}
\end{figure}

\begin{algorithm}[!ht]
\caption{Search(source)}
\begin{algorithmic}
 \State $SegmentList\leftarrow$  source's $SegmentList$ 
 \State $SegmentId\leftarrow0$
 \State $Segment\leftarrow  SegmentList[SegmentId]$
 \State $c\leftarrow Segment's$ $c$ value
\While{($c$ equals to 0)} \Comment {searching for the first $Segment$ with positive $c$ value} 
\State $SegmentId\leftarrow SegmentId+1$
\State $Segment\leftarrow  SegmentList[SegmentId]$
\State $c\leftarrow Segment's$ $c$ value
\EndWhile
create a binary array $S$ of size $ \dfrac{N}{logN}$. Initialize with zeros
\For{\textbf{each} node $n$ in $Segment's$ $eList$}
\State $S[n-(SegmentId-1)\dfrac{N}{logN}]\leftarrow 1$
\EndFor
\For{\textbf{each} node $n$ in $Segment's$ $sList$}
\State $S[n-(SegmentId-1)\dfrac{N}{logN}]\leftarrow 1$
\EndFor
\Comment {searching for the first non probed destination}
\State $destination\leftarrow 1$
\While{($S[destination]$ equals to 1)}  
\State $destination\leftarrow destination+1$
\EndWhile
\State \Return $destination+(SegmentId-1)\dfrac{N}{logN}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Update($source,destination,probing_result$)}
\begin{algorithmic}
\State $segmentIndex\leftarrow  \floor*{\frac{nodeId}{\frac{N}{logN}}}$
\If{($probing_result$ is $s$)}
\State push $destination$ to $source's$ $SegmentList[segmentIndex].sList$
\Else
\State push $destination$ to $source's$ $SegmentList[segmentIndex].eList$
\EndIf
\State decrease $source's$ $SegmentList[segmentIndex].c$ by one
\end{algorithmic}
\end{algorithm}

\begin{flushleft}\textbf{The GSOE algorithm}\end{flushleft}
In the previous subsection we explained how destination nodes are selected from \textit{SegmentList} given a source node. In this subsection we explain the rules that GSOE follows in order to select source nodes. We also describe how probing results affect the graph-level and node-level properties. 

The selection of source node is based on the Switch-On-Empty principal that comes from the original algorithm. When a probing comes up empty the source node should change and another node should act as source. In GSOE this rule in enhanced with other rules.\newline 
\textit{\textbf{Rule 1:}}When a probing comes out solid the s value of source and destination nodes are increased by one.\newline
\textit{\textbf{Rule 2:}}When a probing comes out empty the e and state values of source and destination nodes are decreased by one.\newline
\textit{\textbf{Rule 3:}}A node v can be pushed to TOP list if GSOE found its actual degree (see Lemma 1) and its state equals to zero.\newline
\textit{\textbf{Rule 4:}} When a node has $state$ less than 0 it cannot be selected as source. It can only be selected as destination node. A node v can be selected as source if only has state 0 and does not fulfill \textit{Rule 3}.\newline

GSOE terminates when TOP list is filled with the TOP-K degree nodes. The following lemma provides a way to identify when the top-K degree nodes have been identified.


\textit{\textbf{Lemma 2:}} Nodes with same degree are pushed to TOP list during the same round or equivalently nodes that are pushed during the same round have the same degree.\\
\textit{\textbf{Proof:}} 
Assume that two nodes $u$,$v$ are pushed to TOP during the same round. This means that GSOE spent the same number of rounds until it pushes them to TOP. Based on Lemma 2 we conclude that:\\
$e(u)+1 = e(v)+1 \implies e(u)=e(v)$ (1)\\
Since $u$ and $v$ are in TOP it implies that:\\
$s(u)+e(u)$=$N-1$ (2)\\
$s(v)+e(v)$=$N-1$ (3)\\
From (2) and (3) it implies that\\
$s(u)+e(u)$ = $s(v)+e(v)$ (4)\\
From (1),(4) it comes that $s(u) = s(v)$

Having Lemma 2 in mind, we could say that if at the end of a round there's a number of nodes in TOP equal or greater than K then GSOE must terminate and not proceed to a next round.  

\begin{algorithm}[H]
\caption{GSOE(G(V,E),K)}
\begin{algorithmic}
\State $N\leftarrow  \left|V\right|$  
\Comment {N is the number of nodes}
\While{nodes exist in G}
	\Comment {A new round starts}
    \If{(Number of nodes in TOP list \geqslant K)}
     	\State exit
    \EndIf 
    \State $source\leftarrow$ the first node with zero state  
    \While{($source.s$+$source.e$ = $N$-1)} 
    	\State push $source$ to $TOP$
        \Comment {see Rules 3 and 4}
        \State $source\leftarrow$ the next node with zero state
    \EndWhile
    \While{($source\leqslant$ last node in G)} 
    	\State $destination\leftarrow$ $Search(source)$
        \State $result \leftarrow probing(source \rightarrow destination)$
        \State $Update(source,destination,result)$
        \State $Update(destination,source,result)$
 		\If{($result$ is $solid$)}
    		\State Increase $source.s$ by one
            \State increase $destination.s$ by one
            \Comment {see Rule 1}            
            \If{($source.s$+$source.e$ = $N$-1)}
            	\State Push $source$ to $TOP$
                \Comment {see Rule 3}               
            \EndIf
            \If{($destination.s$+$destination.e$ = $N$-1 and destination.state is zero)}
            	\State Push $destination$ to $TOP$
                \Comment {see Rule 3}          
            \EndIf            
  		\Else
    		\State Increase $source.e$ by one
            \State Increase $destination.e$ by one
            \State Decrease $source.state$ by one
            \State Decrease $destination.state$ by one
            \Comment {see Rule 2}
            \State $source\leftarrow$ the next node with zero state 
  		\EndIf 
    \EndWhile     
\EndWhile
\end{algorithmic}
\end{algorithm}

\textit{\textbf{Lemma 3:}} $\forall u \notin TOP,e(u)+1 =$ Number of GSOE rounds spent with u not in TOP.\\
\textit{\textbf{Proof:}}
From the $state$ definition we conclude that when $e$ is increased by one then $state$ is decreased by one too. This means that a node u's $state$ is decreased e(u) times. According to Rule 3, GSOE pushes a node to TOP if only this node has zero $state$. Recall that a negative $state$ value is increased by one at the end of each round. So for a node u that is pushed to TOP it applies that:  
$e(u)+1$ = Number of GSOE rounds performed and $u$ still not in TOP. \\
In case that a node $u$ is one of the TOP-K degree nodes at the end of GSOE it comes that:
$e(u)+1$ = Number of GSOE rounds needed to push the node to TOP. 

\begin{figure}[H]
\begin{center}
\begin{minipage}{4cm}
\centerline{\epsfig{file=figs/example.eps,height=4cm,width=13cm}}
\end{minipage}
\end{center}
\caption{One round is needed if K=1. 2 rounds are needed if K=2. We have a gain of 20 percent in both cases.}
\end{figure}


\begin{flushleft}\textbf{An example}\end{flushleft}
Consider the graph G in Fig.4. We present a GSOE execution in cases looking the TOP-1 and TOP-2 degree nodes. Graph G has 5 nodes (N=5) and thus the maximum number of probings is 10. We'll show that GSOE needs less than 10 probings to reveal TOP-1 and TOP-2 degree nodes.

\textit{Case K=1:} GSOE selects node 1 as source node and searches its SegmentList for destination candidates. It probes destination node 2 which is the first node that node 1 hasn't probed yet. The result is 'S' which means that the s counters of both nodes are increased and their state remains zero. The SegmentLists of nodes 1 and 2 are updated in order to avoid further probings between these nodes in the future. Since the last probing was solid, the source node remains the same and all we need is a new destination node. Obviously the next destination nodes  are 3 and 4 which result to solid probings as well. After the first 3 probings, the s values for nodes 1,2,3,4 are 3,1,1,1 respectively. The next destination node is 5 which is the first empty probing so far. Since the result is 'E' the e values for nodes 1 and 5 are increased by one and their state becomes -1. The switch-on-empty principal orders that GSOE should search for a new source node. Under the condition that a new source node must have zero state (Rule 4) the next source is node 2. Node 2 searches its SegmentList as well and the first non probed destination candidate is node 3. This probing comes up 'E' and consequently the e values for both nodes become 1 and their states decrease to -1. The switch-on-empty rule applies again and triggers the selection of a new source node. The next suitable source is node 4. Node 3 is bypassed because its state became negative after the last probing. The process keeps going with the probings: (4$\,\to\,$2,4$\,\to\,$3,4$\,\to\,$5). Since node 4 performed all possible probings and fulfills the condition: s+e = N-1 and its state is zero (Rule 3), GSOE pushes this node to TOP-list. Whenever a node is pushed to TOP, GSOE checks if TOP-K query has been answered. After the removal of node 4, N-1-minEinG becomes 3 and minDegreeInTOP becomes 4. According to the Terminate function this inequality enables the increment of variable dinstictDegreesInTOP to 1. Since dinstictDegreesInTOP equals to K, GSOE stops after 8 probings! We have a gain of 20 percent since maximum number of probings is 10. In the experimental results we'll show that the gain of probings is quite bigger for bigger graphs and becomes ever bigger if user provides GSOE with a K value that is relatively large compared to the number of nodes in graph.  

\textit{Case K=2:} In this case, dinstictDegreesInTOP is 1 and since it is less than K further probings will be needed. In the continuation of GSOE the next source node would be node 5 which probes node 2 getting an 'E' result and the switch-on-empty rule apples. At this point GSOE check if it has performed a full round over the graph nodes and there's no other node to select as source.i.e no node fulfills Rule 4 preconditions. This means that it is time to increase by one all the negative states in order for GSOE to be able to search for proper source nodes in a new round. The increment of negative states results to the second table in Fig.4. where node 4 is missing (pushed to TOP) and the states of all nodes have become zero again. At the beginning of the second round, GSOE checks node 1 in order to select it as source but the algorithm also sees that node 1 fulfills the condition: s+e=N-1 and its state is 0 (Rule 3). GSOE pushes node 1 to TOP and checks if it should terminate. After the pushing node 1, minDegreeInTOP becomes 3 and N-1-minEinG becomes 2.This inequality causes the increment of dinstictDegreesInTOP from 1 to 2. Now GSOE terminates because now dinstictDegreesInTOP=K=2. We see that GSOE did not perform further probings to find TOP-2 degree nodes!  

\begin{flushleft}\textbf{CoreGSOE: problem definition}\end{flushleft}
In this section we propose the CoreGSOE algorithm to deal with the K-Core detection problem in Hidden Graphs. Given a graph G and a user-defined integer K, our algorithm takes advance of GSOE and searches for cores of order K (K-Core) in G. In case CoreGSOE finds that K-core(s) exists it returns the nodes that compose the core(s), otherwise it returns a boolean false value. Again our aim is to find the K-Core(s) performing as less probings as possible.\\

\begin{flushleft}\textbf{CoreGSOE-The algorithm:}\end{flushleft}
In GSOE, the user-defined integer K is the number of nodes that user wishes to learn about their degree. The same does not apply in case of CoreGSOE where K is the order of core that user wishes to find in the hidden graph. Having the core definition in mind, we propose CoreGSOE. Our algorithm slightly modifies GSOE in order to filter the nodes and select only those nodes that may compose a core of order K. The following two criteria reveal CoreGSOE rationale.\\

Selection Condition:\\
In order for a node to belong to a K-core its degree should be at least equal to K. After an empty probe CoreGSOE estimates the maximum degree value that source and destination nodes could reach. For this purpose CoreGSOE introduces a new node-level parameter called $PotentialDegree$. In a graph G with N nodes it applies that $\forall u \in G, PotentialDegree(u)=N-1-e(u).$ If a node's $PotentialDegree$ becomes less than K then CoreGSOE blacklists this node. This practically means that probings from or towards this node are useless and thus the blacklisted node will never be chosen again to act either as source or destination node.\\
It is easy to calculate a node's $PotentialDegree$. When a probing between two nodes comes up empty their $e$ values increase by one and consequently their $PotentialDegree$ are decreased by one. Note that a node's final $PotentialDegree$ equals to its actual degree when there are no probings left for them. In such a case for a node $u$ applies that $s(u)=PotentialDegree(u)=deg(u)$\\ 
Termination-Condition-A:\\
From core definition we conclude that in order for a graph to have a K-core there must be at least K+1 nodes with degree greater or equal to K. Once CoreGSOE realizes that it is impossible to find at least K+1 nodes with degree greater or equal to K ,it returns a false result meaning that the graph does not contain a K-Core. CoreGSOE introduces a new variable, $PotentialCoreNodes$, to monitor the number of nodes that may compose a K-Core. Assuming that at the start of the algorithm all nodes may belong to a K-Core, $PotentialCoreNodes$ is initialized to |V|. As described above, $PotentialDegree$ gets decreased after an empty probe. Once $PotentialDegree$ becomes less than K then $PotentialCoreNodes$ gets decreased by one too. Due to Termination-Condition-A, when $PotentialCoreNodes$ value gets dropped under K+1 a K-Core does not exist and as a result CoreGSOE returns false.\\
Termination-Condition-B:\\
Termination-Condition-A cannot restrict the number of probes in the positive case where $PotentialCoreNodes$ is equal or larger than K+1. Assume that GSOE evolves and the number of nodes pushed to TOP list has become already equal or larger than K+1. This means that $PotentialCoreNodes$ will never drop under K+1. Thus CoreGSOE will terminate once all probes are performed (N/(N-1)/2).  To deal with this case we introduced a new variable called $MaxPotentialDegree$. $MaxPotentialDegree$ is the maximum $PotentialDegree$ among nodes that haven't been pushed to TOP yet. At the end of each round we check the value of $MaxPotentialDegree$ and if it is less than K then we know that there's no node in G that fulfills the Selection Condition. Obviously there's no need to search among nodes in G and perform further probes. This condition, Termination-Condition-B, helps in dealing with the above problematic case where Termination-Condition-A is not enough.\\
One could say that using Termination-Condition-B as the only termination criterion for CoreGSOE is enough. This is true. Checking if $MaxPotentialDegree$ is less than K at the end of each round indicates if all nodes with $PotentialDegree$ larger or equal to K have been identified or not. Unfortunately Termination-Condition-B can be applied only at the end of a round where the final value $MaxPotentialDegree$ is known since all nodes have been met. The benefit of Termination-Condition-A is that it is applied after each empty probe and immediately finds if $PotentialDegreeNodes$ becomes less than K+1. In such case we will not expect the end of GSOE round to check $MaxPotentialDegree$ and possibly avoid more unnecessary probes.   
\\
NOTE: CoreGSOE does not calculate the following GSOE parameters:
$minDegreeInTOP$,$minEinG$,$dinstictDegreesInTOP$,$mpd$.\\


\begin{algorithm}[H]
\caption{CoreGSOEUpdate(Node u,int K)}
\begin{algorithmic}
\State $PotentialDegree(u)\leftarrow N-1-e(u)$
\If{( PotentialDegree(u) \geqslant K)}
	\If{( $PotentialDegree(u)$ > $MaxPotentialDegree$  )}
		\State $MaxPotentialDegree\leftarrow PotentialDegree(u)$
        \Comment {MaxPotentialDegree is initialized to 0 when a new round starts}
	\EndIf
\Else
	\State $PotentialCoreNodes--$
    \Comment {PotentialCoreNodes equals to |V|=N at the start of GSOE}
	\If{( $PotentialCoreNodes$ < $K+1$  )}
		\State $Return false$
		\Comment {Criterion 2: Core does not exist}        
	\EndIf	
\EndIf
\end{algorithmic}
\end{algorithm}

Source node selection:\\
CoreGSOE traverses over the nodes following the GSOE rules so it comes that the algorithm select a source node if only its state is zero. Criterion 1 adds one more selection criterion.    

\begin{algorithm}[H]
\caption{CoreGSOE(G(V,E),K)}
\begin{algorithmic}
\State $N\leftarrow  \left|V\right|$  
\Comment {N is the number of nodes}
\State $PotentialCoreNodes\leftarrow  N$ 
\Comment {PotentialCoreNodes is the number of nodes than can compose a K-Core}
\State $MaxPotentialDegree\leftarrow  N-1$ 
\Comment {MaxPotentialDegree is the max degree of the nodes that haven't pushed to TOP yet.}
\While{nodes exist in G}
   	\If{(MaxPotentialDegree < K)}
   		\State return CoreDecomposition(TOP)
   	\EndIf
    \State $u\leftarrow  the first node with zero state AND PotentialDegree(u) \geqslant K$
    \Comment {Criterion 1}
	\While{(s(u)+e(u)=N-1)}
    	\State push u to TOP
        \State $u\leftarrow next node with zero state and PotentialDegree(u) \geqslant K$
    \EndWhile    
    
    \State $MaxPotentialDegree\leftarrow 0$
	\While{(u $\leqslant$ last node in G))}
		\State $proberesult \leftarrow probe(u,v)$
        \State $Update(u,v,probe_result)$
		\State $Update(v,u,probe_result)$ 
        \If{(proberesult = empty)}
        	\State Increase e(u) by one
			\State Increase e(v) by one
			\State decrease state(u) by one
			\State decrease state(v) by one
            \If{(CoreGSOEUpdate(u,K) = false)}
            \Comment Criterion 2
            	\State CoreGSOE exits returning false
            	\Comment K-core does not exist.
            \EndIf
            \If{(CoreGSOEUpdate(v,K) = false)}
            \Comment Criterion 2
            	\State CoreGSOE exits returning false 
            	\Comment K-core does not exist.            
            \EndIf 
            \While{(v is not NULL)}
            	\State $u\leftarrow next node with zero state and PotentialDegree(u) \geqslant K$
            	\State v = CoreGSOESDestSearch(u)
            \EndWhile
        \Else
        	\State Increase s(u) by one
			\State Increase s(v) by one
            \If{(s(v)+e(v) = N-1)}
            	\State push v to TOP
            \EndIf            
            \If{(s(u)+e(u) = N-1)}
            	\State push u to TOP
                \State $u\leftarrow next node with zero state and PotentialDegree(u) \geqslant K$
            \EndIf    
        \EndIf
    \EndWhile         
\EndWhile
\end{algorithmic}
\end{algorithm}


\begin{flushleft}\textbf{An example}\end{flushleft}
\begin{figure}[H]
\begin{center}

\begin{minipage}{4cm}
\centerline{\epsfig{file=figs/MAXCORE.eps,height=10cm,width=9cm}}
\end{minipage}

\end{center}
\caption{Max core of order 3 has been detected before performing probe 4->5.}
\end{figure}
